ORORA: Outlier-Robust Radar Odometry

Radar sensors are emerging as solutions for perceiving surroundings and estimating ego-motion in extreme weather conditions. Unfortunately, radar measurements are noisy and suffer from mutual interference, which degrades the performance of feature extraction and matching, triggering imprecise matching pairs, which are referred to as outliers. To tackle the effect of outliers on radar odometry, a novel outlier-robust method called \textit{ORORA} is proposed, which is an abbreviation of \textit{Outlier-RObust RAdar odometry}. To this end, a novel decoupling-based method is proposed, which consists of graduated non-convexity~(GNC)-based rotation estimation and anisotropic component-wise translation estimation~(A-COTE). Furthermore, our method leverages the anisotropic characteristics of radar measurements, each of whose uncertainty along the azimuthal direction is somewhat larger than that along the radial direction. As verified in the public dataset, it was demonstrated that our proposed method yields robust ego-motion estimation performance compared with other state-of-the-art methods. Our code is available at https://github.com/url-kaist/outlier-robust-radar-odometry.

==> section/results_and_discussion.tex <==
% \vspace{-0.3cm}
\section{Experimental Results}
% \vspace{-0.15cm}

In our experiments, we compared our ORORA with other feature-based state-of-the-art methods. To this end, three types of RANSAC proposed in~\cite{burnett2021we} are used: \textcolor{rvc}{the} original RANSAC~\cite{fischler1981ransac} without any compensation, \textcolor{rvc}{MC-RANSAC} whose motion distortion is compensated~\cite{burnett2021we}, and \textcolor{rvc}{MC-RANSAC + \texttt{DPLR}} that both motion and Doppler distortions are compensated\cite{burnett2021we}. For a fair comparison, we used the official open-source implementations. To closely examine the performance of ego-motion estimation depending on the quality of feature extraction, two feature extraction methods proposed in~\cite{cen2018precise} and \cite{cen2019radar} were tested, which are referred to as \texttt{Cen2018} and \texttt{Cen2019}, respectively.


\begin{comment}
\begin{figure}[t!]
	\captionsetup{font=footnotesize}
	\centering 
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=1.0\textwidth]{figs/ts_perc_error.eps}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=1.0\textwidth]{figs/rot_per_100m_error.eps}
		\caption{}
	\end{subfigure}
	\vspace{-0.15cm}
	\caption{Performance changes in terms of (a) relative translation error and (b)~relative rotation error with respect to the ratio of noise bound and voxel size in \texttt{DCC03} of MulRan dataset~\cite{kim2020mulran}.}
	\label{fig:vox_nb_ablation}
\end{figure}
\end{comment}



\begin{figure}[t!]
	\centering 
	\begin{subfigure}[b]{0.50\textwidth}
		\includegraphics[width=1.0\textwidth]{figs/uncertainty_tendency.pdf}
	\end{subfigure}
	\captionsetup{font=footnotesize}
	\caption{Translation error with respect to the size of the radial and azimuthal uncertainties of each feature point~(best viewed in color).}
	\label{fig:a-cote}
\end{figure}


\input{table/w_wo_a_cote.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Performance Changes With Respect to Uncertainty}

First, performance changes in terms of radial and azimuthal uncertainties were analyzed. Interestingly, the different tendency was observed depending on the environments, as shown in Fig.~\ref{fig:a-cote}. It was shown that larger azimuthal uncertainty leads to significant performance improvement in obstructed environments which include more buildings and consist of narrow roads. The experimental results can be interpreted that the larger azimuthal uncertainty enables to suppress the potential errors caused by the feature points located closely on the lateral side, i.e. along the $y$-axis of the sensor frame. That is, these points are likely to have larger uncertainty along the $x$-axis due to their azimuthal uncertainties. % Consequently, performance is significantly improved, as shown in~Table~\ref{table:w_wo_a_cote}. 

In contrast, smaller azimuthal uncertainty showed better performance in wide-opened environments. This is because the features are relatively evenly distributed, so the feature points located on the lateral side are relatively distant from the sensor frame. \textcolor{rvc}{For this reason}, our A-COTE shows comparable performance with the case where anisotropic modeling is not employed, i.e. COTE~\cite{lim2022quatro}, \textcolor{rvc}{in \texttt{Riverside03}}, as shown in Table~\ref{table:w_wo_a_cote}. 

% Therefore, we selectively set the radial and azimuthal uncertainties based on the characteristics of the surroundings.

\textcolor{rvc}{Therefore, it was demonstrated that our A-COTE is more effective in complex urban environments.}  

 
 \subsection{Comparison With the State-of-the-Art Methods}
 
 \begin{figure*}[t!]
 	\centering 
 	\begin{subfigure}[b]{0.92\textwidth}
 		\includegraphics[width=1.0\textwidth]{figs/overall_traj_v4.pdf}
 	\end{subfigure}
 	\vspace{-0.1cm}
 	\captionsetup{font=footnotesize}
 	\caption{Qualitative comparison with the state-of-the-art methods depending on the feature extraction methods, namely, \texttt{Cen2018}~\cite{cen2018precise} and \texttt{Cen2019}~\cite{cen2019radar}, in MulRan dataset~\cite{kim2020mulran}. $\Box$ and $\times$ marks denote start and end points, respectively~(best viewed in color).}
 	\label{fig:overall_traj}
 	\vspace{-0.2cm}
 \end{figure*}
 
 \input{table/mulran_table_all_fine_tuning.tex}

 In general, the state-of-the-art methods showed precise odometry results, overcoming the effect of outliers. However, our ORORA showed more significant performance, as shown in Fig.~\ref{fig:overall_traj} and Table~\ref{table:mulran_comparison}. In particular, it is noticeable that no matter what feature extraction method was used, our ORORA outputs the most precise odometry performance. Therefore, it can be concluded that our ORORA is less sensitive to the performance of feature extraction methods. 
 
 Furthermore, it was observed that our ORORA is more robust against the featureless scenes. In MulRan dataset, sequences captured on the riverside and Sejong city have fewer geometrical characteristics because these scenes are wide-opened environments, so the feature extraction and matching results output less number of feature pairs and a larger ratio of outliers within the correspondences. Under that circumstance, the state-of-the-art methods showed larger performance degradation than ORORA. In addition, it was shown that once the odometry estimation becomes imprecise, the Doppler compensation occasionally rather deteriorates the odometry performance (see the performance difference of MC-RANSAC and MC-RANSAC + \texttt{DPLR}). 
 
 Therefore, these experimental results demonstrate that our ORORA is the most robust method in that our proposed method tolerates the effect of outliers and the performance of ORORA is more invariant to the quality of the estimated correspondences as well. 
 
 
 


\subsection{Algorithm Speed}
 \vspace{-0.1cm}
 
Furthermore, our ORORA is available in real-time, as presented in Fig.~\ref{fig:alg_time}. The speed of ORORA depends on the number of feature pairs, and it \textcolor{rvc}{just} took 5.63 msec on average. The whole pipeline runs at  11.5~Hz, which is sufficiently faster than the frequency at which a radar image is acquired, i.e. 4 Hz.

\begin{figure}[t!]
    \centering
	\begin{subfigure}[b]{0.187\textwidth}
		\includegraphics[width=1.0\textwidth]{figs/time_scatter_hr.png}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{0.263\textwidth}
		\includegraphics[width=1.0\textwidth]{figs/time_stacked_hr.png}
		\caption{}
	\end{subfigure}
	\vspace{-0.15cm}
	\captionsetup{font=footnotesize}
	\caption{(a) Time taken for pose estimation with respect to the number of correspondences\textcolor{rvc}{. The average time is indicated by the black dashed line (Avg: 5.63 msec).} (b)~Area plot of computation time of each module on Intel(R) Core i7-7700K in \texttt{KAIST03} of the MulRan dataset~\cite{kim2020mulran}. As a feature extraction method, \texttt{Cen2019}~\cite{cen2019radar} was exploited~(best viewed in color).}
	\label{fig:alg_time}
    \vspace{-0.6cm}
\end{figure}

==> table/ablation_table.tex <==
\begin{table}[h]
    \centering
    \caption{Performance comparison based on the presence or absence of each component of ORORA in \texttt{DCC03} in MulRan dataset~\cite{kim2020mulran}~($t_\text{rel}$ and $r_\text{rel}$: relative translation and rotation errors, respectively).}
	\setlength{\tabcolsep}{5pt}
    \begin{tabular}{ccccc}
		\toprule \midrule
	Voxelization & A-ROT     & A-COTE &  $t_\text{rel}$ [$\%$] &  $r_\text{rel}$ [$\deg / 100 $m]  \\ \midrule
	            &            &           &          4.93 &       1.52      \\  
	 \checkmark &            &           &          2.80 &       0.73      \\  
     \checkmark & \checkmark &           &          2.40 &       0.58      \\  
     \checkmark &            &\checkmark &          - &       - \\ 
     \checkmark & \checkmark &\checkmark &          - &       - \\ \midrule \bottomrule
	\end{tabular}
	\label{table:csfa}
\end{table}


==> table/comparison_w_PhaRaO.tex <==

\begingroup
\begin{table}[t!]
    \captionsetup{font=footnotesize}
	\centering
	\caption{Comparison with \textit{PhaRao}, which is a renowned direct radar odometry method. The quantitative results of PhaRao are from \cite{park2020pharao}~($t_\text{rel}$:~\%, $r_\text{avg}$:~$\deg$).}  
	% \setlength{\tabcolsep}{4pt}
	{\scriptsize
	
	\begin{tabular}{l|cccccc}
	
	\toprule \midrule
	\multirow{2}[3]{*}{Method} & \multicolumn{2}{c}{\texttt{DCC02}} & \multicolumn{2}{c}{\texttt{KAIST03}} & \multicolumn{2}{c}{\texttt{RIV02}} \\  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
	 & $t_{\text{rel}}$ & $r_{\text{rel}}$ & $t_{\text{rel}}$ & $r_{\text{rel}}$ & $t_{\text{rel}}$  & $r_{\text{rel}}$   \\ \midrule
	 PhaRaO~\cite{park2020pharao}     & 1.91 & 0.234 & \textbf{2.75} & 0.178 &  2.36 &  0.466  \\ 
	 ORORA (Ours)                     &   -  &   - &  3.49 & \textbf{0.12} &   - &   -   \\ 
	\midrule\bottomrule
	\end{tabular}
	}
	\label{table:comparison_w_pharao}
% 	\vspace{-0.15cm}
\end{table}
\endgroup

==> table/mulran_table_all.tex <==

\begingroup
\begin{table*}[t!]
    \captionsetup{font=footnotesize}
	\centering
	\caption{Comparison of odometry test with the state-of-the-art methods on MulRan KITTI dataset~\cite{geiger2012kitticvpr}. The results of deep learning-based methods are from \cite{fischer2021stickypillars,li2020dmlo} ($t_\text{rel}$:~\%, $r_\text{rel}$:~$\deg$/100m).}  
	\vspace{-0.15cm}
	{\scriptsize
	
	\begin{tabular}{l|l|cccccccccc}
	
	\toprule \midrule
	&\multirow{2}[3]{*}{Method} & \multicolumn{9}{c}{Sequence} & \multirow{2}[3]{*}{Mean}\\  \cmidrule(lr){3-11}
	&  & DCC01 & DCC02 & DCC03 & KAIST01 & KAIST02 & KAIST03 & Riverside01 & Riverside02 & Riverside03 &   \\ \midrule
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2018}}}} & RIGID~\cite{besl1992method} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\
 	&RANSAC~\cite{burnett2021we} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\
 	&RANSACMdDoppler~\cite{burnett2021we} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m  & a/b \\
 	&ORORA~(Ours) & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\\midrule
 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2019}}}} & RIGID~\cite{besl1992method} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\
 	&RANSAC~\cite{burnett2021we} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\
 	&RANSACMdDoppler~\cite{burnett2021we} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m  & a/b \\
 	&ORORA~(Ours) & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\\midrule
 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{ORB}}}} & RIGID~\cite{besl1992method} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\
 	&RANSAC~\cite{burnett2021we} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\
 	&RANSACMdDoppler~\cite{burnett2021we} & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m  & a/b \\
 	&ORORA~(Ours) & a/b & c/d & e/f & g/h & j/k & l/m & g/h & j/k & l/m & a/b \\
 	\midrule \bottomrule
	\end{tabular}
	}
	\label{table:kitti_comparison}
	\vspace{-0.15cm}
	
\end{table*}
\endgroup

==> table/mulran_table_all_original.tex <==

\begingroup
\begin{table*}[t!]
    \captionsetup{font=footnotesize}
	\centering
	\caption{Comparison of odometry test with the state-of-the-art methods on MulRan dataset~\cite{kim2020mulran}. }%The bold and the gray-highlight denote the best and the second-best performance, respectively~($t_\text{rel}$:~\%, $r_\text{rel}$:~$\deg$/100m). }  
	\vspace{-0.15cm}
	\setlength{\tabcolsep}{5pt}
	{\scriptsize
	\begin{tabular}{l|l|cccccccccc}
	\toprule \midrule
	&\multirow{2}[3]{*}{Method} & \multicolumn{10}{c}{Sequence} \\  \cmidrule(lr){3-12}
	&  & \texttt{DCC01} & \texttt{DCC02} & \texttt{DCC03}  & \texttt{KAIST02} & \texttt{KAIST03} & \texttt{RIV01} & \texttt{RIV02} & \texttt{RIV03} &  \texttt{Sejong02} & \texttt{Sejong03}   \\ \midrule
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2018}}}} & 
 	RANSAC                     &5.56/1.43  &5.39/1.83    & 10.32/3.38 
 										&12.09/3.56& 19.14/4.53 
 										&32.05/7.59&12.45/3.29& 7.31/2.21 
 										&      */*         & 16.83/3.36  \\
 	&MD-RANSAC               &8.87/2.64&3.76/1.00& 6.09/1.84 
 											&6.67/1.96& 9.19/2.46 
 											&16.37/4.60&16.03/3.92& 7.72/2.19 
 											&8.93/2.11 & 11.30/2.10 \\
 	&MD-RANSAC + \texttt{DPLR}    &9.41/2.90&3.64/1.00& 6.11/1.83 
 															&7.26/2.20& 6.85/1.93 
 															&100.74/4.61&76.68/1.94& 6.61/1.88 
 															&9.84/2.20 & 11.34/2.04 \\
 	&ORORA~(Ours)              & \hl{3.18/\textbf{0.66}} & \hl{\textbf{2.30}/0.57} & \hl{2.77/0.79} 
 	                            &\hl{\textbf{3.12/0.78}} & \hl{\textbf{2.53/0.57}}
 	                            & \hl{\textbf{3.51/0.76}} & \hl{3.31/0.76} & \hl{2.79/0.64} 
 	                            & \hl{3.76/\textbf{0.67}} & \hl{5.07/0.86} \\ \midrule
 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2019}}}} &
 	RANSAC                  &5.41/1.39&4.16/1.07& 3.66/1.06 &4.60/1.39& 6.13/1.56 &3.99/0.96&3.54/0.98& 4.23/1.11 &4.83/1.18& 8.65/1.66  \\
 	&MD-RANSAC              &4.17/0.95&3.14/0.66& 2.70/0.67 &3.46/1.00& 3.31/0.99 &3.83/1.07&3.61/1.03& 3.94/0.96 &4.43/1.01& 6.62/1.12 \\
 	&MD-RANSAC + \texttt{DPLR} &4.01/0.89&2.87/\hl{\textbf{0.55}} & 2.70/0.66 &3.59/1.08& 3.60/1.05 &4.12/1.13&3.93/1.11& 3.81/0.92 &4.51/1.01& 6.55/1.13 \\
 	&ORORA~(Ours)           &\hl{\textbf{3.12}/0.67} & \hl{2.64}/0.63 & \hl{\textbf{2.37/0.57}} 
 	                        &\hl{3.28/0.82} & \hl{3.04/0.70} 
                            &\hl{3.53/0.84}& \hl{\textbf{2.69/0.66}} & \hl{\textbf{2.11/0.49}} 
                            &\hl{\textbf{3.36}/0.81} & \hl{\textbf{4.23/0.73}} \\ \midrule \bottomrule
	\end{tabular}
	}
	\label{table:kitti_comparison}
	\vspace{-0.15cm}
	
    % \vspace{-0.15cm}
\end{table*}
\endgroup

==> table/mulran_table_v2.tex <==

\begingroup
\begin{table}[t!]
    \captionsetup{font=footnotesize}
	\centering
	\caption{Comparison of odometry test with the state-of-the-art methods on MulRan dataset~\cite{geiger2012kitticvpr}. }%The bold and the gray-highlight denote the best and the second-best performance, respectively~($t_\text{rel}$:~\%, $r_\text{rel}$:~$\deg$/100m). }  
	\vspace{-0.15cm}
	\setlength{\tabcolsep}{3pt}
	{\scriptsize
	\begin{tabular}{l|l|cccc}
	\toprule \midrule
	&\multirow{2}[3]{*}{Method} & \multicolumn{4}{c}{Sequence} \\  \cmidrule(lr){3-6}
	&  & DCC03 &  KAIST03 & Riverside03 & Sejong03   \\ \midrule
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2018}}}} & 
 	RANSAC                     & 10.32/3.38 & 19.14/4.53 & 7.31/2.21 & 16.83/3.36  \\
 	&MD-RANSAC                 & 6.09/1.84 & 9.19/2.46 & 7.72/2.19 & 11.30/2.10 \\
 	&MD-RANSAC + \texttt{DPLR}    & 6.11/1.83 & 6.85/1.93 & 6.61/1.88 & 11.34/2.04 \\
 	&ORORA~(Ours)              & \hl{3.07/0.97} & \hl{\textbf{2.88/0.73}} & \hl{2.78/0.76} & \hl{5.31/0.95} \\ \midrule
 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2019}}}} &
 	RANSAC                  & 3.66/1.06 & 6.13/1.56 & 4.23/1.11 & 8.65/1.66  \\
 	&MD-RANSAC              & 2.70/0.67 & 3.31/0.99 & 3.94/0.96 & 6.62/1.12 \\
 	&MD-RANSAC + \texttt{DPLR} & \hl{\textbf{2.70/0.66}} & 3.60/1.05 & 3.81/0.92 & 6.55/1.13 \\
 	&ORORA~(Ours)           & 2.73/0.72 & \hl{2.94/0.81} & \hl{\textbf{2.56/0.78}} & \hl{\textbf{3.93/0.80}} \\ 
 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\midrule \bottomrule
	\end{tabular}
	}
	\label{table:kitti_comparison}
	\vspace{-0.15cm}
	
    % \vspace{-0.15cm}
\end{table}
\endgroup

==> table/mulran_table_w_orb.tex <==

\begingroup
\begin{table}[t!]
    \captionsetup{font=footnotesize}
	\centering
	\caption{Comparison of odometry test with the state-of-the-art methods on MulRan dataset~\cite{geiger2012kitticvpr}. }%The bold and the gray-highlight denote the best and the second-best performance, respectively~($t_\text{rel}$:~\%, $r_\text{rel}$:~$\deg$/100m). }  
	\vspace{-0.15cm}
	\setlength{\tabcolsep}{3pt}
	{\scriptsize
	\begin{tabular}{l|l|cccc}
	\toprule \midrule
	&\multirow{2}[3]{*}{Method} & \multicolumn{4}{c}{Sequence} \\  \cmidrule(lr){3-6}
	&  & DCC03 &  KAIST03 & Riverside03 & Sejong03   \\ \midrule
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{ORB}}}} & 
	RANSAC                  & 5.58/1.62 & 12.67/3.79 & 5.89/1.54 & 9.26/1.63  \\
 	&MD-RANSAC              & 5.36/1.54 & 11.34/3.47 & 6.29/1.52 & 9.54/1.72 \\
 	&MD-RANSA C+ \texttt{D} & 5.08/1.49 & 7.39/2.21 & 6.13/1.62 & 9.31/1.66 \\
 	&ORORA~(Ours)           & 5.46/1.60 & 12.82/3.95 & 5.96/1.61 & 8.37/1.45 \\ \midrule
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2018}}}} & 
 	RANSAC                     & 10.32/3.38 & 19.14/4.53 & 7.31/2.21 & 16.83/3.36  \\
 	&MD-RANSAC                 & 6.09/1.84 & 9.19/2.46 & 7.72/2.19 & 11.30/2.10 \\
 	&MD-RANSAC + \texttt{D}    & 6.11/1.83 & 6.85/1.93 & 6.61/1.88 & 11.34/2.04 \\
 	&ORORA~(Ours)              & \hl{3.07/0.97} & \hl{\textbf{2.88/0.73}} & \hl{2.78/0.76} & \hl{5.31/0.95} \\ \midrule
 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\texttt{Cen2019}}}} &
 	RANSAC                  & 3.66/1.06 & 6.13/1.56 & 4.23/1.11 & 8.65/1.66  \\
 	&MD-RANSAC              & 2.70/0.67 & 3.31/0.99 & 3.94/0.96 & 6.62/1.12 \\
 	&MD-RANSAC + \texttt{D} & \hl{\textbf{2.70/0.66}} & 3.60/1.05 & 3.81/0.92 & 6.55/1.13 \\
 	&ORORA~(Ours)           & 2.80/0.73 & \hl{2.94/0.81} & \hl{\textbf{2.56/0.78}} & \hl{\textbf{3.93/0.80}} \\ 
 	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 	\midrule \bottomrule
	\end{tabular}
	}
	\label{table:kitti_comparison}
	\vspace{-0.15cm}
	
\end{table}
\endgroup
